Do uHear? Validation of uHear App for Preliminary Screening of Hearing Ability in Soundscape Studies

Studies involving soundscape perception often exclude participants with hearing loss to prevent impaired perception from affecting experimental results. Participants are typically screened with pure tone audiometry, the "gold standard" for identifying and quantifying hearing loss at specific frequencies, and excluded if a study-dependent threshold is not met. However, procuring professional audiometric equipment for soundscape studies may be cost-ineffective, and manually performing audiometric tests is labour-intensive. Moreover, testing requirements for soundscape studies may not require sensitivities and specificities as high as that in a medical diagnosis setting. Hence, in this study, we investigate the effectiveness of the uHear app, an iOS application, as an affordable and automatic alternative to a conventional audiometer in screening participants for hearing loss for the purpose of soundscape studies or listening tests in general. Based on audiometric comparisons with the audiometer of 163 participants, the uHear app was found to have high precision (98.04%) when using the World Health Organization (WHO) grading scheme for assessing normal hearing. Precision is further improved (98.69%) when all frequencies assessed with the uHear app is considered in the grading, which lends further support to this cost-effective, automated alternative to screen for normal hearing.

==> [ICA22] uHear Validation 2/table/cfstats.tex <==
\begin{table}[t]
\caption{Accuracy, sensitivity, specificity, and precision, and McNemar's Test \textit{p}-value of the WHO and WHO+ grading criteria for normal hearing. WHO+ includes the measurements at 6 kHz in the grading, which is on top of the 4 frequencies in the WHO grading (i.e. 0.5, 1, 2, and \SI{4}{\kilo\hertz}).}
\centering
\begin{tabularx}{\textwidth}{lc*{3}{>{\centering\arraybackslash}X}c}
\toprule
Grading                     &   
Accuracy (\%; \SI{95}{\%} CI)  &   
Sensitivity (\%)            &   
Specificity (\%)            &   
Precision (\%)              &
MNT \textit{p}-value            \\

\midrule
WHO                     &   
95.09 (90.56, 97.86)        &   
96.77                       &   
62.50                       &   
98.04                       &
0.723                       \\

WHO+                           &   
98.16 (94.72, 99.62)        &   
99.34                       &   
81.82                       &   
98.69                       &
1.000                        \\
\bottomrule
\end{tabularx}
\label{tab:cfmetrics}
\end{table}

==> [ICA22] uHear Validation 2/table/wrs.tex <==
\begin{table}[t]
\centering
\caption{Wilcoxon signed rank tests, and the pseudomedian and its confidence intervals (\SI{}{\decibel} HL; 95\% confidence level) of the differences between the audiometer and uHear audiograms are computed at each frequency (0.5, 1, 2, 4 and \SI{6}{\kilo\hertz}) across both ears. The null hypothesis is rejected at \textit{p}-value $<0.05$.}
\setlength{\tabcolsep}{12pt}
\begin{tabularx}{\textwidth}{%
    X
    S[table-format=1.1]
    S[table-format=-1.1]
    r@{\hskip0pt}S[table-format=-1.1,table-space-text-pre={[}]
    @{,\hskip-35pt}S[table-format=-1.1]<{{)}}
    S[table-format=1.2e2]}
\toprule
Ear & {Frequency (\si{\kilo\hertz})} & {Pseudomedian} & \multicolumn{3}{c}{Confidence Interval (\SI{95}{\%})\qquad}  & \multicolumn{1}{c}{\textit{p}-value}\\
\midrule
\multirow{5}{*}{\centering\arraybackslash Left}
& 0.5 & -5.0 &\qquad(&-5 & -5& 6.11e-7\\

& 1 & -7.5  &\qquad(&-7.5 & -7.5& 3.37e-19\\

& 2 & -5.0  &\qquad(&-7.5 & -2.5& 7.14e-7\\

& 4 & -5.0  &\qquad(&-7.5 & -5& 1.65e-10\\

& 6 & 2.5  &\qquad(&0 & 5& 1.13e-3\\
    
\midrule
\multirow{5}{*}{\centering\arraybackslash Right}
& 0.5 & -5.0  &\qquad(&-5 & -2.5& 2.14e-6\\

& 1 & -7.5  &\qquad(&-7.5 & -7.5& 4.31e-23\\

& 2 & -5.0  &\qquad(&-7.5 & -5& 1.61e-13\\

& 4 & -7.5  &\qquad(&-7.5 & -7.5& 1.67e-16\\

& 6 & 2.5  &\qquad(&0 & 2.5& 6.82e-2\\
\bottomrule
\end{tabularx}
\label{tab:wrs_results}
\end{table}


